Pruning Deep Neural Networks using Partial Least Squares

Modern pattern recognition methods are based on convolutional networks since they are able to learn complex patterns that benefit the classification. However, convolutional networks are computationally expensive and require a considerable amount of memory, which limits their deployment on low-power and resource-constrained systems. To handle these problems, recent approaches have proposed pruning strategies that find and remove unimportant neurons (i.e., filters) in these networks. Despite achieving remarkable results, existing pruning approaches are ineffective since the accuracy of the original network is degraded. In this work, we propose a novel approach to efficiently remove filters from convolutional networks. Our approach estimates the filter importance based on its relationship with the class label on a low-dimensional space. This relationship is computed using Partial Least Squares (PLS) and Variable Importance in Projection (VIP). Our method is able to reduce up to 67% of the floating point operations (FLOPs) without penalizing the network accuracy. With a negligible drop in accuracy, we can reduce up to 90% of FLOPs. Additionally, sometimes the method is even able to improve the accuracy compared to original, unpruned, network. We show that employing PLS+VIP as the criterion for detecting the filters to be removed is better than recent feature selection techniques, which have been employed by state-of-the-art pruning methods. Finally, we show that the proposed method achieves the highest FLOPs reduction and the smallest drop in accuracy when compared to state-of-the-art pruning approaches. Codes are available at: https://github.com/arturjordao/PruningNeuralNetworks

==> Sections/RelatedWork.tex <==
\section{Related Work}\label{sec:relatedwork}
%The idea in pruning networks is to find neurons that could be removed without degrading its original performance. To this end, several works have proposed different approaches to identify the potential neurons to be removed. In particular, most existing pruning approaches focus on eliminating neurons (filters) in convolutional layers since $99\%$ of overall FLOPs are concentrated on these layers~\cite{Han:2015}.
%
To find unimportant filters, Hu et al.~\cite{Hu:2016} proposed to observe the percentage of zeros activations (APoZ) in the resulting feature map from a filter (coupled with ReLU activation). The idea behind the method is that filters which yield feature maps with large APoZ are redundant and could be removed. In their method~\cite{Hu:2016}, once APoZ from all filters have been computed, the ones larger than one standard deviation are eliminated and the resulting network is fine-tuned. Hu et al.~\cite{Hu:2016} demonstrated that measuring the APoZ considering all layers, decreases network accuracy considerably and it is hard to recover its original performance, therefore, their method is executed layer-by-layer. Similar to~\cite{Hu:2016}, Li et al.~\cite{Li:2017} proposed to discard filters based on its magnitude. For this purpose, the authors compute the L1-norm from each filter and remove the filters with small magnitudes. Since filters coming from {different} layers present different magnitude orders, their L1-norms cannot be compared directly to decide which filters to remove. As a consequence, the approach of Li et al.~\cite{Li:2017} prunes the network considering one layer at the time followed by a fine-tune of the entire network. A notable drawback in their work is the requirement of human efforts to test different tradeoffs between the pruning rate and the network performance.

Different from the hand-crafted pruning criteria employed in~\cite{Hu:2016, Li:2017}, Huang et al.~\cite{Huang:2018} proposed a data-driven pruning method. Their method eliminates redundant filters by learning agents, which are encouraged to remove a large number of filters while preserving the network performance above a threshold. According to results presented by Huang et al.~\cite{Huang:2018}, for each agent (which is responsible for pruning a single layer) around $150$ training iterations are necessary for convergence. In addition, after pruning a layer, some stages of fine-tuning are performed on the entire network. As a consequence, their method is unfeasible in deep networks.
{Similar to Huang et al.~\cite{Huang:2018}, He et al.~\cite{He:2018} proposed a pruning strategy based on agents that learn to penalize accuracy loss and encourage model compression. These agents can employ different policy search protocols: (i) latency, where resulting network has the best accuracy given an amount of hardware resources and (ii) quality, where the output network is the smallest as possible with no loss of accuracy. We show that our method is able to achieve both criteria and is also more accurate.}

To address the problem of eliminating neurons layer-by-layer, Yu et al.~\cite{Yu:2018} proposed to remove the filters coming from all layers at once. {To this end, the authors applied the Infinity Feature Selection~\cite{Roffo:2015} method on the final layer output to obtain the importance of each neuron. Then, this importance is recursively propagated throughout the network using a proposed neuron score propagation algorithm. Finally, neurons with low importance are removed and the network is fine-tuned.}
%To this end, the authors applied the Infinity Feature Selection method on the final response layer to obtain the importance of each neuron. Then, this importance is recursively propagated throughout the network using a proposed neuron score propagation algorithm. Finally, neurons with low importance are removed and the network is retrained.

In contrast to most existing pruning approaches~\cite{Hu:2016, Li:2017, Huang:2018}, our method is able to remove filters from different layers at once. Therefore, it performs few fine-tuning stages, which makes the method extremely efficient. {Additionally, since the PLS can be learned using few samples (e.g., $10\%$ of training samples), our method is computationally efficient. We emphasize that this fact is an advantage of the PLS regarding the other dimensionality reduction and feature selection techniques applied to prune, such as Singular Value Decomposition (SVD)~\cite{Denton:2014, Girshick:2015}, Principal Component Analysis (PCA)~\cite{Wang:2018} and infinity feature selection~\cite{Yu:2018}.}
Finally, due to our effective pruning criterion, we achieve a higher reduction in FLOPs (without degrading the network performance) than existing pruning techniques~\cite{Hu:2016, Li:2017, Huang:2018, Yu:2018}.
